AutoBench: Automatic Testbench Generation and Evaluation Using LLMs for HDL Design

In digital circuit design, testbenches constitute the cornerstone of simulation-based hardware verification. Traditional methodologies for testbench generation during simulation-based hardware verification still remain partially manual, resulting in inefficiencies in testing various scenarios and requiring expensive time from designers. Large Language Models (LLMs) have demonstrated their potential in automating the circuit design flow. However, directly applying LLMs to generate testbenches suffers from a low pass rate. To address this challenge, we introduce AutoBench, the first LLM-based testbench generator for digital circuit design, which requires only the description of the design under test (DUT) to automatically generate comprehensive testbenches. In AutoBench, a hybrid testbench structure and a self-checking system are realized using LLMs. To validate the generated testbenches, we also introduce an automated testbench evaluation framework to evaluate the quality of generated testbenches from multiple perspectives. Experimental results demonstrate that AutoBench achieves a 57% improvement in the testbench pass@1 ratio compared with the baseline that directly generates testbenches using LLMs. For 75 sequential circuits, AutoBench successfully has a 3.36 times testbench pass@1 ratio compared with the baseline. The source codes and experimental results are open-sourced at this link: https://github.com/AutoBench/AutoBench

==> Acknowledgement.tex <==
% \begin{acks}
\section*{Acknowledgment}
This work is supported by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) -Project-ID 504518248 and by TUM International Graduate School of Science and Engineering (IGSSE).

% \end{acks}

==> Reference.tex <==
% \printbibliography

\let\oldbibliography\thebibliography
\renewcommand{\thebibliography}[1]{%
\oldbibliography{#1}%
\fontsize{8.5pt}{8.5}\selectfont
\setlength{\itemsep}{0.03pt}%
}

%\setlength{\labelsep}{-3pt}
% \newpage
\normalem
% \bibliographystyle{IEEEtran}
% %\bibliographystyle{ACM-Reference-Format}
% \bibliography{ref}


\bibliographystyle{ACM-Reference-Format}
\bibliography{ref}

==> codes/code_python_checker.tex <==
% python block

% verilog block



\begin{promptbox}{}\tiny

%%%%%%%%%%%%%%%%%%%%%%%%%%%%stage 3%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textcolor{red}{\textbf{Stage3}}:

\textcolor{cyan}{\textbf{\acronym{}}}:

1. Your task is to write a verilog testbench for a verilog RTL module code ... 

2. you are in stage 3; in this stage, please give me the core rules of an ideal DUT ...

...\textcolor{teal}{(\omitted)}

3. your information is:

\textbf{[problem description]}

\textbf{[testbench specification from Stage 1]}

\textbf{[test scenarios from stage 2]}

your response should only contain python code. For convenience, you can use binary or hexadecimal format in python. For example: 0b0010 and 0x1a
    
\textcolor{violet}{\textbf{LLM}}:

Here's the Python code which will provide the expected results based on the input vector provided to each scenario.

\lstvspacetop
\lstinputlisting[language=Python, style=python-style]{codes/stage3_code.v}
\lstvspacebottom

\hspace*{\fill}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%stage 5%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textcolor{red}{\textbf{Stage5}}:

\textcolor{cyan}{\textbf{\acronym{}}}:

Your task is ... \textcolor{teal}{(\omitted)}

\textbf{[DUT header]}

\textbf{[problem description]}

\textbf{[scenario list from stage 2]}

\textbf{[beginning of desired testbench]} \textcolor{teal}{(generated from DUT header)}

... \textcolor{teal}{(\omitted)}

\textcolor{violet}{\textbf{LLM}}:

% ... \textcolor{teal}{(\omitted)}

\lstvspacetop
\lstinputlisting[language=Python, style=python-style]{codes/stage5_code.v}
\lstvspacebottom

\end{promptbox}

==> codes/code_verilog_driver.tex <==
% python block

% verilog block


\begin{promptbox}{}\tiny

%%%%%%%%%%%%%%%%%%%%%%%%%%%%stage 2%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textcolor{red}{\textbf{Stage2}}:

\textcolor{cyan}{\textbf{\acronym{}}}:

1. Your task is to write a verilog testbench for a verilog RTL module code ... \textcolor{teal}{(\omitted)}

2. you are in section2 ...\textcolor{teal}{(\omitted)}

3. your information is:

\textbf{[problem description]}:

Build a combinational circuit with 100 inputs, in[99:0]. There are 3 outputs: 

// (1) out\_and: output of a 100-input AND gate. 

// (2) out\_or: output of a 100-input OR gate. 

// (3) out\_xor: output of a 100-input XOR gate.


\textbf{[testbench specification from \textbf{Stage 1}]}:

\{``important data": ``",
  
  ``technical specifications": [
    ``1. DUT Module Description: The Device Under Test (DUT) is defined in the Verilog module named `top\_module'. It contains a single input bus of width 100 bits (in[99:0]) and three separate output signals: out\_and, out\_or, and out\_xor. These outputs represent the computed AND, OR, and XOR operations of all 100 inputs respectively.",
    
    ``2. ...", ...
     ]\} \textcolor{teal}{(\omitted)}
    
\textcolor{violet}{\textbf{LLM}}:

\{
  ``scenario 1": ``All input bits are set to 0 (000...000). This tests the basic operation when all inputs are at their lowest value.",
  
  ``scenario 2": ``All input bits are set to 1 (111...111). This scenario checks the outputs when all inputs are at their maximum.",
  
  ``scenario 3": ``Alternating bits starting with 0 (0101...01). This pattern is essential to examine how the circuit handles alternating values.",

  ... \textcolor{teal}{(\omitted)}
\}

\hspace*{\fill}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%stage 4%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textcolor{red}{\textbf{Stage4}}:

\textcolor{cyan}{\textbf{\acronym{}}}:

Your task is ... \textcolor{teal}{(\omitted)}

\textbf{[DUT header]}

\textbf{[problem description]}

\textbf{[scenario list from stage 2]}

\textbf{[beginning of desired testbench]} \textcolor{teal}{(generated from DUT header)}

... \textcolor{teal}{(\omitted)}

\textcolor{violet}{\textbf{LLM}}:

% ... \textcolor{teal}{(\omitted)}

\lstvspacetop
\lstinputlisting[language=Verilog,style=verilog-style]{codes/stage4_code.v}
\lstvspacebottom

\end{promptbox}

==> codes/codes_baseline.tex <==
\begin{promptbox}{Prompt of Baseline}\scriptsize
    Your task is to write a verilog testbench for an verilog RTL module code (we call it as ``DUT", device under test). The infomation we have is the problem description that guides student to write the RTL code (DUT) and the header of the ``DUT".
    
    [code format template]
    
    [problem description]
    
    [DUT header in verilog]
    
    very very IMPORTANT: If all the test cases passed, the testbench should display ``all test cases passed". If any one of the test cases failed, testbench should not display ``all test caess passed". DO NOT generate any .vcd file.
    please don't reply other words except the testbench codes.
\end{promptbox}


==> codes/stages/Stage4SEQ.tex <==
\databoxbegin{stage4SEQ}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textcolor{cyan}{\textbf{Prompt}:}

1. Your task is to complete a given verilog testbench code. This testbench is for a verilog RTL module code (we call it as ``DUT", device under test). This circuit is a \textbf{sequential circuit}. ...\textcolor{teal}{(\omitted)}\\

Your information is:

[\textbf{problem description} from \textbf{Benchmark Suite}]

[\textbf{module header} from \textbf{Benchmark Suite}] 

[\textbf{testbench specification} from \textbf{Stage 1}]

[\textbf{scenario list} from \textbf{stage 2}]\\

The testbench does not need to check the DUT's output but only exports the signals of the DUT. Please export the signals of DUT to a file named ``TBout.txt" at the end of each scenario. The template is given below:\\
\$fdisplay(file, ``[check]scenario: \%d, clk = \%d, load = \%d, ena = \%d, amount = \%d, data = \%d, q = \%d", scenario, clk, load, ena, amount, data, q);\\
The variables are already declared. The clock signal is already prepared. This output will be used to check the correctness of the DUT's output later.\\
Please only use ``\#10" as the delay when needed. If you need a longer delay, you can use multiple ``\#10", such as ``\#10; \#10; \#10;". Avoid meaningless long delays in your code.\\

...\textcolor{teal}{(\omitted)}\\

Please determine the input signal's exact values according to the test scenarios. \\
Note: please complete the last initial code part (marked in the given testbench template). You should give me the completed full code. The testbench template above is to help you generate the code. You must use \%d when exporting values.\\
Please generate the full testbench code. please only reply Verilog codes, no other words. \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textcolor{orange}{\textbf{LLM’s Output}:}

\codevspacetop
\lstinputlisting[language=Verilog, style=verilog-style]{codes/stage4SEQ_code.v}
\codevspacebottom\\
\vspace{0.3cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textcolor{cyan}{\textbf{Prompt}:}

Please help me to export the input of DUT module by using code below:

[IMPORTANT]:
\$fdisplay(file, ``scenario: \%d, clk = \%d, load = \%d, ena = \%d, amount = \%d, data = \%d, q = \%d", scenario, clk, load, ena, amount, data, q);

You should insert the code above into scenario checking part. In each scenario, you should insert the code above after the input of DUT module changed. Don't delete the existing \$display codes.

For example, for a circuit that has two input signals changed at different times in one scenario, the original code is like this:
- original code:
// scenario 1 begins\\
scenario = 1;\\
signal\_1 = 1; \\
// insert \$fdisplay here\\
\#10; \\
signal\_2 = 1; \\
// insert \$fdisplay here\\
\#10; \\
\$fdisplay(file, ``[check]scenario: \%d, clk = \%d, load = \%d, ena = \%d, amount = \%d, data = \%d, q = \%d", scenario, clk, load, ena, amount, data, q);\\
#10;\\
// scenario 1 ends\\
...\textcolor{teal}{(\omitted)}

Please insert codes according to the rules above. DO NOT modify other codes! Please reply with the modified full codes. please only reply with Verilog codes, no other words.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textcolor{orange}{\textbf{LLM’s Output}:}

\codevspacetop
\lstinputlisting[language=Verilog, style=verilog-style]{codes/stage4bSEQ_code.v}
\codevspacebottom\\

\databoxend{}


==> latexmkrc <==
@default_files = ("main_tex.tex");

$bibtex_use = 2;
$pdf_mode = 1;
$pdflatex='pdflatex -synctex=1 %O %S';

add_cus_dep('vsz', 'pdf', 0, 'veusz_pdf' );
sub veusz_pdf {
system( "/Applications/Veusz.app/Contents/MacOS/veusz.exe --export=\"$_[0].svg\" --export-option=svgtextastext=True \"$_[0].vsz\"" );
return system( "inkscape -D --export-type=pdf --export-filename=\"$_[0].pdf\" \"$_[0].svg\"" ); 
}

add_cus_dep('svg', 'pdf', 0, 'inkscape_pdf' );
sub inkscape_pdf {
return system( "inkscape -D --export-type=pdf --export-filename=\"$_[0].pdf\" \"$_[0].svg\"" ); 
}

